Affinity-Graph-Guided Contractive Learning for Pretext-Free Medical Image Segmentation with Minimal Annotation

The combination of semi-supervised learning (SemiSL) and contrastive learning (CL) has been successful in medical image segmentation with limited annotations. However, these works often rely on pretext tasks that lack the specificity required for pixel-level segmentation, and still face overfitting issues due to insufficient supervision signals resulting from too few annotations. Therefore, this paper proposes an affinity-graph-guided semi-supervised contrastive learning framework (Semi-AGCL) by establishing additional affinity-graph-based supervision signals between the student and teacher network, to achieve medical image segmentation with minimal annotations without pretext. The framework first designs an average-patch-entropy-driven inter-patch sampling method, which can provide a robust initial feature space without relying on pretext tasks. Furthermore, the framework designs an affinity-graph-guided loss function, which can improve the quality of the learned representation and the model generalization ability by exploiting the inherent structure of the data, thus mitigating overfitting. Our experiments indicate that with merely 10% of the complete annotation set, our model approaches the accuracy of the fully annotated baseline, manifesting a marginal deviation of only 2.52%. Under the stringent conditions where only 5% of the annotations are employed, our model exhibits a significant enhancement in performance surpassing the second best baseline by 23.09% on the dice metric and achieving an improvement of 26.57% on the notably arduous CRAG and ACDC datasets.

==> Tables/modules.tex <==
% \begin{table}[!h]
% \centering
% \caption{Ablation study of $\mathcal{L}^{RW}_{AGG}$ and $\mathcal{L}^{PL}_{AGG}$ on ACDC dataset.}
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{*{9}{c|}c}
% \toprule
% \multicolumn{2}{c|}{Module}                                            & \multicolumn{4}{c|}{Label=5\%} &\multicolumn{4}{c}{Label=10\%}\\ \hline
% $\mathcal{L}^{RW}_{AGG}$ & $\mathcal{L}^{PL}_{AGG}$ & DSC$\uparrow$ &Jacard$\uparrow$ & HD95$\downarrow$ & ASD$\downarrow$ & DSC$\uparrow$ & Jacard$\uparrow$ & HD95$\downarrow$ & ASD$\downarrow$ \\ \midrule
% \checkmark              &                         &               &                  &                  &               &               &                  &                  &               \\ \hline
%                         & \checkmark              &               &                  &                  &               &               &                  &                  &               \\ \hline
% \checkmark              & \checkmark              &               &                  &                  &               &               &                  &                  &               \\ \bottomrule
% \end{tabular}}
% \end{table}


\begin{table*}[ht]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{*{13}{c|}c}
\toprule
\multicolumn{3}{c|}{$\mathcal{L}^{PL}_{AGG}$}                                                                   & \multicolumn{3}{c|}{$\mathcal{L}^{RW}_{AGG}$}                                                & \multicolumn{4}{c|}{Label=5\%}                                                                                 & \multicolumn{4}{c}{Label=10\%}                                                                                \\ \hline
\multicolumn{1}{c|}{w/GK+L2} & \multicolumn{1}{c|}{w/GK+L1} & \multicolumn{1}{c|}{w/ $\lambda||\mathbf{A}||*$} & \multicolumn{1}{c|}{$A_{ii}$} & \multicolumn{1}{c|}{1:1} & \multicolumn{1}{c|}{random} & \multicolumn{1}{c|}{DSC} & \multicolumn{1}{c|}{Jacard} & \multicolumn{1}{c|}{HD95} & \multicolumn{1}{c|}{ASD} & \multicolumn{1}{c|}{DSC} & \multicolumn{1}{c|}{Jacard} & \multicolumn{1}{c|}{HD95} & \multicolumn{1}{c}{ASD} \\ \midrule
-                           & -                           & -                           & -          & -          & -          &     &        &      &     &     &        &      &     \\ \hline
\multirow{8}{*}{\checkmark} & \multirow{8}{*}{}           & \multirow{4}{*}{}           &            &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             & \checkmark &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            & \checkmark &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            &            & \checkmark &     &        &      &     &     &        &      &     \\ \cline{3-14} 
                            &                             & \multirow{4}{*}{\checkmark} &            &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             & \checkmark &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            & \checkmark &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            &            & \checkmark &     &        &      &     &     &        &      &     \\ \hline
\multirow{8}{*}{}           & \multirow{8}{*}{\checkmark} & \multirow{4}{*}{}           &            &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             & \checkmark &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            & \checkmark &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            &            & \checkmark &     &        &      &     &     &        &      &     \\ \cline{3-14} 
                            &                             & \multirow{4}{*}{\checkmark} &            &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             & \checkmark &            &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            & \checkmark &            &     &        &      &     &     &        &      &     \\ \cline{4-14} 
                            &                             &                             &            &            & \checkmark &     &        &      &     &     &        &      &     \\ \hline
\end{tabular}}
\end{table*}

% \begin{table}[ht]
% \caption{Ablation study of different ratio in $\mathcal{L}^{RW}_{AGG}$ on ACDC dataset}
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \toprule
% \multirow{2}{*}{$\mathcal{L}^{RW}_{AGG}$} & \multicolumn{4}{c|}{Label=5\%}& \multicolumn{4}{c}{Label=10\%}\\ \cline{2-9} 
% & \multicolumn{1}{c|}{DSC$\uparrow$} & \multicolumn{1}{c|}{Jacard$\uparrow$} & \multicolumn{1}{c|}{HD95$\downarrow$} & ASD$\downarrow$ & \multicolumn{1}{c|}{DSC$\uparrow$} & \multicolumn{1}{c|}{Jacard$\uparrow$} & \multicolumn{1}{c|}{HD95$\downarrow$} & ASD$\downarrow$ \\ \midrule
% w/o RW&               &                  &                  &               &               &                  &                  &               \\ \hline
% $A_{ii}$ ratio&               &                  &                  &               &               &                  &                  &               \\ \hline
% fix 0.5 ratio&               &                  &                  &               &               &                  &                  &               \\ \hline
% random ratio&               &                  &                  &               &               &                  &                  &               \\ \bottomrule
% \end{tabular}}
% \end{table}
